Fast and Scalable Analysis of Massive Social Graphs

Graph analysis is a critical component of applications such as online social networks, protein interactions in biological networks, and Internet traffic analysis. The arrival of massive graphs with hundreds of millions of nodes, e.g. social graphs, presents a unique challenge to graph analysis applications. Most of these applications rely on computing distances between node pairs, which for large graphs can take minutes to compute using traditional algorithms such as breadth-first-search (BFS). In this paper, we study ways to enable scalable graph processing on today's massive graphs. We explore the design space of graph coordinate systems, a new approach that accurately approximates node distances in constant time by embedding graphs into coordinate spaces. We show that a hyperbolic embedding produces relatively low distortion error, and propose Rigel, a hyperbolic graph coordinate system that lends itself to efficient parallelization across a compute cluster. Rigel produces significantly more accurate results than prior systems, and is naturally parallelizable across compute clusters, allowing it to provide accurate results for graphs up to 43 million nodes. Finally, we show that Rigel's functionality can be easily extended to locate (near-) shortest paths between node pairs. After a one- time preprocessing cost, Rigel answers node-distance queries in 10's of microseconds, and also produces shortest path results up to 18 times faster than prior shortest-path systems with similar levels of accuracy.

==> append.tex <==
\appendix
\appendixpage
\addappheadtotoc
\section{Related Work}


==> comp.tex <==
\begin{table}[t]
\centering
\begin{tabular}{|c|c c c c|}
\hline
Embedding Space & Euclidean Space(GNP) & Orion & Pisces & Sphere\\
\hline
ARE & 0.17 & 0.15 & 0.09 & 0.36
AER & 0.89 & 0.95 & 1.00 & 0.89
ACR & 1.18 & 1.09 & 1.01 & 1.81
ASPD & 1.23 & 1.19 & 1.10 & 2.03
SD & 12009 & 80 & 45 & 167835
\hline
\end{tabular}
\caption {Evaluate different embedding spaces with different metrics in India graph }
\label{tab:indmet}
\end{table}

ARE: average relative error
AER: average expansion ratio
ACR: average contraction ratio
ASPD: average symmetric pair distortion
SD: space distortion

\begin{figure}[t]
\centering
   \includegraphics[scale=0.65]{figures/ind-metric-dir.eps}
   \caption{CDF of Directional pair distortion under different
     embedding space in India graph}
   \label{fig:inddir}
\end{figure}




\begin{algorithm}
\caption{Cascade Input Order with $n$ $1$-hop local landmarks.}
%\label{alg:1hop} 
\begin{algorithmic}
\STATE //Input: Distances between nodes and landmarks; Neighbors of nodes
\STATE //Output: $k$ neighbors with at most $n$ 1-hop friends
\STATE //Decide nodes input order based on their distances to landmarks
\FOR {each node}
\STATE Find its smallest distances to landmarks;
\STATE Set this distance as its input level $l$;
\ENDFOR

\FOR {each level}
\STATE node in this level will randomly join system;
\STATE node select at most $k$ neighbors from all its neighbors with coordinates;
\ENDFOR
\end{algorithmic}\label{cascade}
\end{algorithm}



==> hyb.tex <==
\section{Combining Two Coordinate Sets}
In the previous section we found that the accuracy on short and 
long distance is in some sense complementary; indeed,
by maximizing the accuracy of short distance estimation we enlarge 
the error on long distance estimation and vice versa.

Here we take a different approach to achieve the same goal, which is 
to find a method that concurrently optimize 
for both short and long distance, here we propose an hybrid approach. 
In particular, we aim to fuse {\em two coordinate sets}
so that  we preserve the accuracy on long distance estimation meanwhile 
improving the short distance estimation. 
%We propose to use a is optimized on short distance estimation and the second 
%on the long distance estimation.
In such a design we would like to combine the advantage of the two sets of coordinates
without paying the price of loosing accuracy on some other distance.
 For convenience, we call the set of coordinates meant to improve 
 short distances as {\bf S-Coordinates}, which are the coordinates derived 
 from the {\em 4 Local Landmarks} method, and the 
 set of coordinates meant to improve long distance as {\bf L-Coordinate}
 which are the coordinates derived from the {\em No Local Landmarks} method.
We propose to estimate the actual distance by leveraging the Maximum 
Likelihood Analysis which help us to derived the unknown real distance 
of a pair of nodes by analyzing the confidence each method provides given a
certain output from the coordinates distance computation. 


\subsection{Hybrid Approach}
The investigation presented in the previous section spun the intuition 
of merging the two methods to simultaneously maintain their benefits. 	
We intend to leverage the confidence of both methods on their estimated distances 
 in order to provide our final distance estimation.  
In the remain of this section we first formally introduce our Hybrid method and then 
we present a measurement-based analysis to quantify its goodness. 

\para{Estimate Distances via Maximum Likelihood Analysis.}
In this section we give the technical details to build a 
model that leverages both our previous methods to maximize  
the expectation on the outcome.
Therefore, the objective is to maximize the likelihood of predicting the correct 
distance from the combined probabilities that each of these two methods 
have to guess it correctly. 

Let $\theta$ be the unknown distance that a strategy $A$ and a strategy 
$B$ are trying to identify.    
Let $X_A$ be a discrete random variable such that $P(X_A=x | \theta)$
is the probability that method $A$ output distance $x$ given a read distance $\theta$.
Similarly, let  $X_B$ be a discrete random variable such that $P(X_B=y | \theta)$
is the probability that method $A$ output distance $y$ given a read distance $\theta$.
Thus, given a certain output  $x$ and $y$ respectively from method 
$A$ and $B$ we are interested in identifying 

\begin{small}
\begin{equation}
\hat{\theta} = arg \max_{\theta \in \Theta} \{f(x,y | \theta)=P(X_A=x | \theta)*P(X_B=y | \theta)\}
\end{equation}
\end{small}


The estimator $\hat{\theta}$ represents the distance that maximizes the likelihood of the joint 
distribution of the two stocastic variables $X_A$ and $X_B$, given a true value $\theta$. 
 
Actually, we model the distribution of the random variable $X_A$ to fit the output of the 
{\em No Local Landmarks} method for each given distance $\theta \in [1, 18]$. Similarly we 
fit the variable $X_B$ on the distribution produced by the {\em 4 Local Landmarks} method, again for 
each $\theta \in [1, 18]$ and then we study the maximum likelihood of the estimator $\hat{\theta}$
of their joint distribution for each $\theta \in [1, 18]$.

\begin{figure}[t]
\centering
   \includegraphics[scale=0.65]{figures/egy-mle-bmark-2_4.eps}
   \caption{\fixme{Average absolute error of MLE method in Egypt graphs}}
   \label{fig:egymle}
\end{figure}

\para{Experimental evaluation.} In this section we intend to compare the three best models
investigated so far, with the maximum likelihood-based model presented here.
As we mentioned before and as showed in Figure~\ref{fig:egymle}, No local landmarks method provides a low error on 
distances grater than $3$-hop although it produce a very high error on short distances. 
On the other side $4$ local landmark gets the error extremely 
low on short distances at the price of a sensitive degradation on long distances. 

Between 
these two methods we experienced the $1$ local landmark 
which was a reasonable compromise in reducing the error on short distances 
without any sensitive degradation of the error on long distances. Although 
$1$ local landmark method is a suitable solution we aimed to reduce 
even more the on short distances.

Figure~\ref{fig:egymle} shows that the maximum likelihood-based 
method not only provides a sensitive lower error on short distances but the error on long
distances (i.e.,  $\geq 6$) is almost everywhere the lowest. 
The region where this method is penalized in on distances $\in [3,5]$. 
However, the increase in error that the maximum likelihood-based 
method shows on intermediate paths is something tolerable 
on the application results as we are going to show  in the next section.


%In the following we explore the two techniques to achieve this goal 
%and we present an experimental evaluation which provides evidence of the
%increased accuracy estimation of short distance estimation with minimal degradation of 
%intermediate distances.
%\subsection{Combining Two Coordinate Sets}
%We intend to leverage two sets of coordinates in order to 
%optimize both short and long distance estimation. Ideally, 
%in order to efficiently use two sets of 
%coordinates it should be a priori known when to use which one.
%Because we do not have any information about the real distance between two nodes 
%then we need to identify, only by looking at the coordinate distance estimation 
%between these two sets, which set of coordinates to use.
%
%In order to achieve this goal we follow two steps:
%first, we compute the distance $d_s$ between two nodes by using the set of short distance coordinate  {\bf S-Coordinates};
%second, if the distance $d_s$ is less or equal to a given threshold $t$ we use the result from 
%the  {\bf S-Coordinate}, otherwise we take the distance $d_l$ computed with the long distance coordinate  {\bf L-Coordinates}.
%
%
%%Although 1-hop friends' information can help to reduce the error of 2-hop distance estimation, we notice that the error in 3-hop distance and long distance estimation is much higher compared to the accuracy computed without 1-hop friends. Thus, we would like to combine the advantage of the two sets of coordinates. For conveniece, we call the set of coordinate which is good at short distance estimation as {\bf short coordinate}; the set of coordinate which is accurate in long distance estimation is called as {\bf long coordinate}.In the rest of this section, we will introduce two schemes to combine the advantages of the two coordinates and we call the estimated distances are computed by {\bf hybrid coordinate}. 
%
%
%%This approach uses a threshold $t$ to distinguish the two distances 
%%computed by long coordinates and short coordinate separately. 
%%Because short coordinate distance is good at estimating short distance, 
%%we suppose that if distance $d_s$ computed by short coordinate is 
%%smaller than threshold $t$, the actual path length 
%%should be $d_s$; otherwise, the path is long and distance $d_l$ computed by long coordinate is used.
%%
%% \begin{algorithm}
%% \caption{Naive hybrid scheme}
%% \label{alg:hyb1} 
%% \begin{algorithmic}
%% \STATE $d_s$: distance computed by short coordinates;
%% \STATE $d_l$: distance computed by long coordinates;
%% \STATE $t$: The threshold;
%% \STATE $d$: distance used as the final result
%% \IF {$d_s \leq t$} 
%% \STATE $d = d_s$
%% \ELSE
%% \STATE $d = d_l$
%% \ENDIF
%% \end{algorithmic}
%% \end{algorithm}
%
%It, now, remains to test the impact of the threshold in distinguishing between short and long distances. 
%We varies the threshold from $1.0$ to $4.0$ and we study how it impacts the average 
%relative error on  different graphs. Figure~\ref{fig:thdare} shows that as the threshold increases also 
%the average relative error increases. This happens because a large threshold 
%engages the S-Coordinate set to estimate also intermediate distances, however, as we know from 
%section \$~\ref{sec:1hop}, it is not strongly accurate.
%%enlarges the distance range that short coordinates are in charge of while 
%%the set of S-Coordinate introduces errors into long distances. 
%%Thus, with increase of threshold, more and more long distances computed 
%%by short distance are of high errors but they are used to estimate path length. 
%%This leads to that the accuracy of our system decreases.
%
%%To further validate our intuition we explore how the threshold impact the accuracy of different path lengths. 
%%Secondly, we look into how the threshold impact the accuracy of different path lengths. 
%%Since our focus is on short distance estimation accuracy, 
%Furthermore, Figure~\ref{fig:thd13} shows the impact of the threshold on the average absolute error of 
%-one, two and three- hops distances. 
%As the threshold increases -one and two- hops distances decrease, instead  
%three-hops distance presents an increase from  $0.7$ to $1.3$, with the same argument we made above.
%%that translate in almost more than $1$ hop error. 
%However, because we aim to improve short distance estimation we prefer to slightly penalize  three-hops distances 
%in vantage of -one and two- hops distances. Therefore, we set the threshold as $2.5$ which is the best trade off between 
%-one and two- hops versus three-hops distances. 
%
%%For 2-hop distance, increase of threshold from 1 to 2.5 can improve the accuracy to estimate 2-hop distance. When threshold is more than 2.5, 2-hop distance estimation error can not reduce greatly. However, at the same time, the distance estimation for 3-hop distances increase from 0.7 to 1.3, which is almost more than 1 hop error. This is because since 3 hop is adjacent to long distances, then part of them can be accurately computed by long coordinates instead of short one. But the only threshold emphases on the accuracy of short distance because it only uses long distances while short coordinates is not smaller than it. Thus, the part of 3-hop distances which can be more accurate predicted by long coordinates are still computed by short coordinates. However, when threshold is more than 2.5, absolute error of 3-hop distances becomes stable. So we set threshold as 2.5 which is the best trade off between the 2-hop and 3-hop distances. 
%
%\begin{figure}[t]
%\centering
%   \includegraphics[scale=0.65]{figures/thred-naive-are.eps}
%   \caption{Average relative error of different thresholds}
%   \label{fig:thdare}
%\end{figure}
%
%\begin{figure}[t]
%\centering
%   \includegraphics[scale=0.65]{figures/egy-th-naive-24hop.eps}
%   \caption{Average absolute error of 1,2 and 3-hop distance with different thresholds}
%   \label{fig:thd13}
%\end{figure}
%
%Finally, we compare our threshold based approach to {\em No Local Landmarks} method
%which was the one with the minimum error on intermediate and long disatnces. 
%As reported in Figure~\ref{fig:egythab}  we are successfully able to reduce the 
%error of -one and two-hops distances meanwhile maintaing the same accuracy 
%on long distance estimation although we are still slightly penalized on -three to six- hops distances.
%However, we achieved our goal on short path lengths we still need to improve the medians.
%In the next section we propose a novel strategy which accomplish this goal, i.e. improve the
%average absolute error from -three to six-hops distances.   
%
%%we plot the absolute error for different path lengths in Egypt when threshold are 0 and 2.5 in Figure~\ref{fig:egythab} to see whether the accuracy of long distance estimation is maintained. Compared to the results computed by long coordinate (threshold is 0), our hybrid coordinate scheme can significantly reduce 2-hop distance error from 1.5 to 0.5 while we can still maintain the estimation accuracy of long distance which is more than 5 hops. However, for 4 to 5 hop distance estimation, we only loss 1 hop accuracy, which can make the short and long distances indistinguishable. That is, some applications which need to make difference between short and long distances will not work well, which we will study in Section~\ref{sec:app}. 
%
%\begin{figure}[t]
%\centering
%   \includegraphics[scale=0.65]{figures/egy-th-naive-1.9.eps}
%   \caption{Average absolute error for different path lengths on {\em No Local Landmarks} and  $2.5$.}
%   \label{fig:egythab}
%\end{figure}
%
%\subsection{The Hybrid Coordinates Set}
%In this section we aim to tune our approach of using a double set of coordinates to achieve 
%a low error among all path lengths and in particular reduce the error from -three to six-hops distances.  
%%We propose a scheme which is more sophisticated scheme to hybrid short and long coordinates to improve median distance.
%% Similar to naive scheme, we still use one threshold to judge when to use short or long coordinates. 
%
%We propose a new scheme which distinguishes three different cases:
%%that works as follow:The threshold $t$ is a metric to predict to distinguish short and long distance. There are three different situations:
%first, if the two estimated distances, $d_s$ and $d_l$, are both smaller 
%than the threshold then the real distance can be accurately computed with $d_s$;
%%is a short distance so that short coordinate is used to compute distance; 
%second, if the two estimated distances are both larger than threshold, 
%%which indicates that the real distance is possible long distance,
%then the real distance can be accurately estimate with $d_l$; 
%finally, if the distances computed with the two sets of coordinates are on different side of the threshold 
%then we estimate the real distance as the expected value between $d_s$ and $d_l$ .
%%  3. When short coordinate predicts distance less than threshold meanwhile long coordinate shows that is longer, this means the real distance is in the 
%%confusing range which is about 3 or 4 hops. Thus, both of predictions are reasonable and the system uses the average of the two distances to do 
%%estimation; 4. if the distance computed by short coordinate is longer than the threshold while the distance computed by long one is shorter, both of them 
%%seems inaccurate so that we can only leverage their average to reduce potential error. In our simulation, situation 4 is rare. So the solution is 
%%acceptable. 
%
%% \begin{algorithm}
%% \caption{Sophisticated hybrid scheme}
%% \label{alg:hyb2} 
%% \begin{algorithmic}
%% \STATE $d_s$: distance computed by short coordinates;
%% \STATE $d_l$: distance computed by long coordinates;
%% t\STATE $t$: The threshold;
%% \STATE $d$: distance used as the final result
%% \IF {$d_s \leq t$ and $d_l \leq t$} 
%% \STATE $d = d_s$
%% \ELSIF {$d_s > t$ and $d_l > t$}
%% \STATE $d = d_l$
%% \ELSIF {$d_s \leq t$ and $d_l > t$}
%% \STATE $d = \frac{(d_s+d_l)}{2}$
%% \ELSIF {$d_s > t$ and $d_l \leq t$}
%% \STATE $d = \frac{(d_s+d_l)}{2}$
%% \ENDIF
%% \end{algorithmic}
%% \end{algorithm}
%
%
%We investigate the accuracy of this approach with the following experimental analysis.
%First, we study the impact of the threshold on the accuracy of our system on different graphs. 
%as we show in Figure~\ref{fig:hyb2are}. Similarly to the results we present in Figure~\ref{fig:thdare}, 
%increasing the threshold the accuracy of the system decreases. However, we directly compare 
%with the previous  approach in  Figure~\ref{fig:egyarecom} to prove the benefits which derive
%from this novel scheme. In particular, setting the threshold is $2.5$, the error of our novel scheme is 
%$34$\% less than the previous scheme. 
%This is because this scheme fairly uses the advantage of both coordinates with less bias on
%the short coordinates set in  the previous scheme.
%
%%compared to naive scheme, where we plot the accuracy of Egypt with two schemes in 
%
%
%%Figure~\ref{fig:egyarecom},which plots the accuracy of Egypt with two schems, shows that sophisticated scheme can better protect accuracy of the whole
%% system. For example, when threshold is 2.5, the error of sophisticated scheme is 34\% less than that of naive scheme. This is because this scheme fairly 
%% use the advantage of both coordinates with less bias to short coordinate in naive scheme.
%% Thus, the distances in confusing areas, e.g. 3 hops and 4 hops, can be estimated with the more accurate coordinates or 
%
%%Furthermore, whether this scheme can improve the accuracy of short distance is tested and the result of Egypt graph is shown in Figure~\ref{fig:egysab13}. 
%Figure~\ref{fig:egysab13} shows the improved accuracy of this scheme as function of 
%different threshold on -one, two and three- hops distances;  we provide the result 
%only on the Egypt graph because it is representative of other result as well 
%and because of the space constraints.
% 
%Increasing the threshold the absolute error of two-hops distances reduces. 
%%and with threshold between 2.6 and 3.0, the accuracy stays the same. 
%At the same time, the accuracy of 3-hop distance estimation is maintained. 
%When threshold is between 2.8 and 3.0, the error of three-hops distances gets even less. 
%%This proves that sophisticated scheme can better leverage the advantage of short and long coordinates so as to maintain or even improve the accuracy of 3-hop distances. 
%Thus, a threshold $\in [2.5, 3]$ seems a reasonable choice. 
%%And for other graphs, we could also samples some of distances to heuristically detect the good choice for threshold. 
% 
%%We plot the absolute error of different path lengths of Egypt graph with threshold of 2.5 
%%in Figure~\ref{fig:egydisab2.5} of two schemes. Both schemes can reduce 
%%2-hop distances error. Compared to naive scheme, sophisticated scheme can better 
%%maintain the accuracy of 3, 4 and 5-hop distance. Sophisticated scheme can be as 
%%accurate as the original system as well. 
%
%We plot the absolute error of different path lengths of Egypt graph with threshold of 2.5 
%in Figure~\ref{fig:egydisab2.5} for both schemes. They provide a sensitive reduction of the error  
%on both -one and two- hops distances; Furthermore, the scheme achieve higher accuracy on  
%-three, four and five- hops distances.
%
%%Thus, sophisticated scheme is a better solution to combine the 
%%advantage of short and long coordinates, which can improve the 
%%accuracy of short distance estimation while maintain accuracy of 
%%median and long distance. 
%
%Concluding, this new method allows us to achieve our general goal which was to
%reduce the error on short path lengths meanwhile maintaining low the error on 
%long path lengths.  
%\begin{figure}[t]
%\centering
%   \includegraphics[scale=0.65]{figures/thred-soph-are.eps}
%   \caption{Average relative error of different thresholds of Sophisticated scheme}
%   \label{fig:hyb2are}
%\end{figure}
%
%\begin{figure}[t]
%\centering
%   \includegraphics[scale=0.65]{figures/egy-th-are-com.eps}
%   \caption{Average relative error of Sophisticated and Naive schemes in Egypt graph}
%   \label{fig:egyarecom}
%\end{figure}
%
%
%\begin{figure}[t]
%\centering
%   \includegraphics[scale=0.65]{figures/egy-th-soph-24hop.eps}
%   \caption{Average absolute error of 1,2 and 3-hop distance with different thresholds in Egypt graph}
%   \label{fig:egysab13}
%\end{figure}
%
%
%\begin{figure}[t]
%\centering
%   \includegraphics[scale=0.65]{figures/egy-th-soph-1.9.eps}
%   \caption{Average absolute error of different path lengths of Egypt graph with threshold of 2.5}
%   \label{fig:egydisab2.5}
%\end{figure}


==> hyperbolic2.tex <==
%\section{Testing System Parameters}
%\label{sec:eval}
%In order to build a real embedding system 
%we need to learn how to calibrate its parameters to naturally blend real social graphs 
%into the geometric space. 
%We propose a measurement driven approach to establish the right methodology 
%to fit our Hyperbolic embedding system to real social graphs.
%All our experiments are run on commodity machines which have 2.4GHz,
%four core and 24 GB RAM. 
%
%\para{Real Social Graphs.} We perform our experimental evaluation on four anonymized graphs
%which are networks crawled from Facebook. The statistic
%features of these four graphs are listed in Table~\ref{tab:graphs}; we explore 
%different graphs to prove that the accuracy of our system is 
%not limited to a single dataset and the large sizes considered are necessary to 
%prove first that our system scale and second to differentiate our investigation from previous 
%proposal where the size of the datasets used where sensibly smaller. 
%%accurate for several dataset and scalable on 
%%which shows that the graph is large and tractable for our
%%evaluation. To evaluate the accuracy of our system, we randomly select
%%5000 nodes from each graphs and use their measured distances computed
%%by BFS as ground truth. 
%
%\para{Evaluation Metrics}
%To evaluate the accuracy of different parameters setting in our system, 
%we leverage two simple metrics: average
%relativie error and absolute error for different path length. 
%
%We use only these two metrics because are the most 
%appropriate in understanding the overall performance of the system
%(with the average relative error) and the local accuracy on different path lengths 
%(with the absolute error computed on any path length).
%
%
%%Relative error is the ratio of the
%%difference between estimated distance and measured distance to the
%%measured distance, which is shown in Equation~\ref{eq:re}. To show the accuracy for the whole graph, we
%%compute the mean of relative error to get the average relative
%%error. Thus, the smaller this error is, the more accurate our system
%%is. 
%%
%%To test the accuracy of our system in estimating different path
%%length, we use absolute error. Since distances in graphs are integers
%%while the estimated distances in our system are real number, we need to distinguish different path length using threshold. Thus, if
%%the absolute error of different path length is smaller enough, we can
%%better to identify its actual path length. 
%
%
%
%%\subsubsection{Landmark Selection Startegy}
%%Selecting the proper set of Landmarks is one of the most 
%%challenging point of our system bootstrap.
%%We would like to find the best possible set of Landmarks that for the case of 
%%the shortest path computation are the {\em central nodes}.
%%The massive size of these graphs limits us from the possibilities of compute the 
%%central nodes and so we decide to explore a different approach.
%%As we proposed in our previous work~\cite{orion10} on Euclidean space, 
%%%we studied the scheme to select
%%%landmarks and show some preliminary results of accuracy of coordinate
%%%in Euclidean space. Thus, here we will use the same parameters to
%%%compute coordinate in Hyperbolic space for comparason purpose. We 
%%we select $100$ high degree nodes as possible landmarks. We use the high degree nodes 
%%because the probability that an high degree node is also a central node is much higher 
%%compared to the same probability on law degree nodes.  
%%At this point we select $16$ out of this possible $100$ landmarks to be the one used in the 
%%optimization algorithm. We do so to efficiently computing the optimization function, 
%%meanwhile we achieve the wanted accuracy making sure that the selected landmarks are 
%%at least $2$-hops away from each other~\cite{orion10}.   
%%and any two of them should be at
%%least 2-hop away. 16 of them are used as basic landmarks to determine
%%space. And to maintain the accuracy and efficiency, we use random 16
%%out of 100 landmarks to calibrate the coordinate of each node.
%%
%%We use four annonymized graphs to evaluate the accuracy of our system,
%%which are four networks crawled from Facebook. The statistic
%%characters of the four graphs are listed in Table~\ref{tab:graphs},
%%which shows that the graph is large and tracable for our
%%evaluation. To evaluate the accuracy of our system, we randomly select
%%5000 nodes from each graphs and use their measured distances computed
%%by BFS as ground truth. 
%%
%%All our experiment were run on commordity machines which has 2.4GHz,
%%four core and 24 GB RAM. 
%
%
%\begin{table}
%\begin{small}
%\centering
%\begin{tabular}{| c | c c c|}
%\hline
%Network & Nodes & Edges & Avg. Path Len.\\
%\hline
%Norway & 293K & 5,589K & 4.2\\
%Egypt & 246K & 1,618K & 5.0\\
%Los Angeles & 275K & 2,115K & 5.2\\
%India & 363K & 1,556K & 6.1\\
%\hline
%\end{tabular}
%\caption {\small Properties of Social Graphs}
%\label{tab:graphs}
%\end{small}
%\end{table}
%
%
%
%\subsection{Fitting Parameters to Real Graphs.}
%An Hyperbolic geometric space can assume different features 
%depending on its parameters value. In this section we explore 
%both the curvature of the space and number of coordinates and then 
%we examine the effects of these parameters on the accuracy of the system 
%by studying the precision achieved in estimating different path lengths.
%
%\para{Impact of Curvature.} 
%The curvature $c$ is an important
%parameter to decide the form of the Hyperbolic space. Whether the
%curvature has impact on the accuracy of our system is a crucial question to
%investigate. Thus, we build different Hyperbolic spaces with curvature values $c$
% from $-50$ to $-1$ and we investigate the effect of these curvatures on the accuracy of the distance 
% estimation among nodes over $4$ different social graphs.  
%
%In Figure~\ref{fig:curvature} we plot the curvature values on the 
%$x-$axis and the resulting average relative error on the $y-$axis. 
%Figure~\ref{fig:curvature} reveals two important points:
%first the curvature effects the accuracy of the system as 
%function of the topological structure of the graphs. Indeed, we can 
%note that on Norway, which has $5$ times more edges than the other graphs 
%and the average path length is the shortest, the measured error is the highest. 
%
%Second, although some differences among different graphs there is a 
%common trend, the error decreases as the curvature goes to $-1$. 
%Note that at $x=0$ correspond the error estimation over the Euclidean space.
%Therefore, our Hyperbolic space method can better model
%social network compared to Euclidean space and so we are going to set the 
%curvature to $-1$ for the remaining of this investigation. 
%%the rest of experiment.
%%\fixme{Thus, Hyperbolic space with large curvature can better model
%%social network compared to Euclidean space. And we will use curvature
%%as -1 in the rest of experiment.}
%
%% shows that as the value of curvature increases, the average relative
%%error of our system declines from -50 to -30. There are no obvious
%%difference when the curvature are between -30 and -5. Once the
%%curvature achieves -1, there is a significant improvement in accuracy,
%%from more than 15\% at curvature $k$ to about 10\%, which is about
%%$\frac{1}{3}$ improvement. Because smaller curvature introduces less
%%distortion into Hyperbolic space, this indicates that the distortion in
%%social graphs is not much, although there are some in social
%%networks. 
% 
%\begin{figure}[t]
%\centering
%   \includegraphics[scale=0.65]{figures/radius_mul.eps}
%   \caption{Accuracy of different curvature}
%   \label{fig:curvature}
%\end{figure}
%
%
%\begin{figure}[t]
%\centering
%   \includegraphics[scale=0.65]{figures/dim.eps}
%   \caption{The impact of dimension}
%   \label{fig:dim}
%\end{figure}
%
%\para{The impact of Dimension.} The dimension of a geometric space 
%plays an important role in providing a reasonable level of accuracy 
%in the estimate of distances among nodes; therefore,   we vary the
%dimension parameter from $2$ to $14$ and we study the respective 
%performances on our accuracy metric. Figure~\ref{fig:dim} plots 
%on the $y-$axis the average
%relative error corresponding to different dimensions on the $x-$axis. We also show the best result of Orion which is in India graph in the figure to make comparason.  
%Increasing the number of dimensions of our geometric space, 
%the error decreases from more than $0.2$ to
%about $0.1$, which is about $ 50\%$ improvement. Moreover, we
%notice that after the sharp reduction of error between $2$ dimensions
%and $6$ dimensions, the accuracy of our system stabilizes over the
%increase of dimension. This means that with a low dimension, such as $6$, 
%we can achieve similar accuracy. Compared to the best result in Orion, an Euclidean coordinate system, the accuracy of the four graphs are always higher. This prove that Hyperbolic space can better model Social graphs than Euclidean space again.
%
%From a more system prospective we explore the tradeoff between accuracy 
%and complexity in maintain an high dimensional embedding system.  
%We reduce the complexity of coordinate computation by using 
%$10$-dimension hyperbolic space meanwhile achieving high accuracy.  
%Note that the complexity
%of Simplex Downhill is $O(d \cdot l)$, where $d$ is the number of
%dimension and $l$ is the number of landmarks.
%In the following of this paper we are going to compare the performance of our 
%Hyperbolic space with our previous Euclidean embedding system Orion which also was
%implemented with  $10$ dimensions.
%%\fixme{Considering that we need to do comparison with the best
%%results of Orion of 10 dimension, we still use 10 dimensions in the
%%rest of this paper. .... I think we should have used $6$ dimension. } 

\section{Accuracy of Different Path Lengths} 
In this section we want to explore the goodness of our predicted distances
on different path lengths, by leveraging the best parameters identified in 
the previous paragraphs.  
Different applications on social graphs leverage 
nodes at different distances. For instance, applications that suggest new friends 
compute $2$-hops neighbor search, 
instead applications, like neighborhood function~\cite{anf2002},
explore nodes at long range too. 
%To study how precise our system are in estimating different path
%length. 
In the remaining we experimentally analyze the accuracy of our embedding system 
both on short and on long distance in order to predict the application level precision that we 
can provide with our system. 
We also compare Pisces with our previous embedding system attempt, Orion, which was 
developed on an Euclidean space.  

\para{Long Distances.} In Figure~\ref{fig:hyperab} we show the absolute error
on different path lengths with
-1 curvature in 10-dimension Hyperbolic space compared to the result of India graph computed by Orion. 
Obviously, Pisces can better estimate distance more than 5 hops than Orion. 
That is why Pisces is more accurate than Orion. In this plot we can see
that for path lengths higher than $5$-hops  the absolute error is roughly  $0.5$,
which means that we are able to accurately distinguish paths of length $5$ 
from path of lengths $4$ or $6$.

\para{Short Distances.} Path lengths less than $4$-hops  show an error 
that incrementally increases by decrementing  the path length.  
Consequently it is more difficult to distinguish nodes 
 $2$-hops aways from nodes $3$-hops distants. 
 
The {\em motivation} of the inaccuracy on short path lengths follows this intuition:
with high probability the distance of a nodes from the landmarks,
when its coordinates are computed, is relatively long which means
its coordinate are calibrated with far away nodes and so short distances
gets penalized.  

We validate our intuition through the experiment in Figure~\ref{fig:hyperab}, which reports 
the average absolute error per path lengths on  graphs with slightly different topological properties.
%Let's focus our attention on the
%$2$ and $3$-hop distances of the India graph.
The India graph shows the highest error from  two to four hops distances compared to the other graphs.
Taking a close look at the statistical characteristic of this graph, as reported in Table~\ref{tab:table1}, we notice that
the average path length of India
is larger than other graphs. Therefore, with high probability the distances from landmarks used in 
calibrating coordinates are also
longer which make the short distance estimation even less accurate than other graphs. 

In other word, the lack of information on smaller distances during the coordinates calibration phase
yield an high error, in particular, on  2
and 3-hop distance estimations.
%We plot the absolute error of different path lengths with
%-1 curvature in 10-dimension Hyperbolic space in
%Figure~\ref{fig:hyperab}. Figure~\ref{fig:hyperab} shows that when the
%distances are more than 5 hops, the absolute error are about 0.5,
%which is a good bounds because the adjacent lengths can be
%distinguished well.
% However, for path length less than 4, the
%error are relative high, which about 1 or more. That means, if we want
%to identify 2 hop and 3 hop, there will generate high misunderstanding
%areas. In India graph, the error for 2 and 3-hop distances are even
%higher than others. This is because the average path length of India
%is larger than others, the distances of most pairs of nodes are longer
%so that the distances used in calibrating coordinates are also
%longer. Thus, lack of information of smaller distance, the error of 2
%and 3-hop distances are higher.
The low accuracy of short distance 
estimation was noticed in previous graph embedding systems too, as in~\cite{Crowcroft_IMC05}, although the 
understanding of this phenomenon was not investigated. 
%Previous work in graph embedding \fixme{(references)} shows that
%high error of short distances is an inevitable
%problems in embedding systems. 
In the next section, we first provide a deeper investigation and comprehension of this phenomenon and then
we introduce a novel approach, which we employ in Pisces, 
that we prove effective in strongly mitigating the high error on short distances. 
\begin{figure}[t]
\centering
   \includegraphics[scale=0.65]{figures/disab.eps}
   \caption{Average absolute error of different path lengths}
   \label{fig:hyperab}
\end{figure}

==> localdis.tex <==
\section{Improving Short Distance Estimation}
\label{sec:local}
% \begin{figure}[t]
% \centering
%    \includegraphics[scale=0.65]{figures/egy-est-bmark-pro.eps}
%    \caption{\fixme{Estimated distances distribution with no local landmarks in Egypt graph}}
%    \label{fig:egyestb}
% \end{figure}

% \begin{figure}[t]
% \centering
%    \includegraphics[scale=0.65]{figures/egy-est-nei4-pro.eps}
%    \caption{\fixme{Estimated distances distribution with Cascade 4 local landmarks in Egypt graph}}
%    \label{fig:egyestn}
% \end{figure}

The importance of short distance estimation lays on the need 
of supporting application functionalities.
In social graphs many applications, e.g. nodes recommendation within $n$ hops, 
base their operability on the
knowledge of the set of nodes within a given distance from a target node. 
Furthermore, this given distance is a short distance, i.e. 
two or three hops from a target node. 

%Short distance are important though difficult to predict with high accuracy.
%In social graphs, the $1$-hop
%information can be easily obtained although many applications, e.g.neighborhood function~\cite{anf2002}, 
%are based on the
%knowledge of short distances which are more than $1$-hop.
%Has been confirmed in previous investigations.
%
%Here we aim to achieve better accuracy by exploring different techniques....

%Previous study \fixme{(some
%  references)} shows that there is always high errors of short
%distances introduced by embedding. In social graph, although 1-hop
%information can be easily obtained from the edge information of
%graphs, many applications, e.g.neighborhood function~\cite{anf2002}, are based on the
%knowledge of short distances which are more than 1 hop.

Although, our embedding system achieves a smaller average relative error
compared to other solutions, as for instance~\cite{orion10}, it is still penalized 
on the {\em short distance estimation}, as reported in Figure~\ref{fig:hyperab}.
Embedding systems are known to produce high error on short distances~\cite{Crowcroft_IMC05},
however, at the best of our knowledge, none dived into this problem 
to provide a better understanding and proper guidelines to design embedding algorithms
with no such a problem.
Therefore, we devote this section to the comprehension of how improve
accuracy of short distance estimation. 
In order to achieve this goal we need to ask two fundamental questions:
\begin{itemize}
\item {\em Is the accuracy of Landmark coordinates the source of error in Pisces? }
\item {\em What is the missing information which does not allow Rigel to properly estimate short path lengths?}
\end{itemize}

We provide a measurement-based analysis to answer 
these two important questions.

%Although Rigel can improve the average relative error in graph distance 
%estimation,  the short distance estimation, i.e. 2 and 3 hops which are 
%smaller than average path length~\ref{tab:graphs}, is still not 
%accurate in Figure~\ref{fig:hyperab}. How to improve
%the accuracy of short distance becomes a challenge in our system design.


%\begin{figure}[t]
%\centering
%   \includegraphics[scale=0.65]{figures/landbas.eps}
%   \caption{Accuracy of secondary landmarks with different number of basic landmarks}
%   \label{fig:basic}
%\end{figure}

\begin{figure}[t]
\centering
   \includegraphics[scale=0.65]{figures/landare.eps}
   \caption{Accuracy of different number of basic landmarks}
   \label{fig:basicare}
\end{figure}

\subsection{Proving Landmarks Accuracy}
Our intend to prove that the error on the short distance estimation is 
{\bf not }caused from possible inaccuracy of the landmark coordinates.


% {\bf not }caused from possible inaccuracy of the landmark coordinates.

% Our aim is to provide the basic understand on our system 
% which supports the 
% design rationale we use in the next section to reduce the error on short distance 
% estimation. We intend to prove that the error on the short distance estimation is 
% {\bf not }caused from possible inaccuracy of the landmark coordinates.

%
%to understand how to improve short distance estimation.
%Before going there, we need to test whether the landmark coordinates are the
%cause of error. If landmarks coordinates hold high errors any 
%node that will use those landmarks to compute its coordinate is injected with this error.  

Remember that in our system only the coordinates of $16$ random landmarks, out 
of the $100$ total, are calibrated through the global optimization algorithm~\cite{simplex}. 
Note that we named {\em primary} landmarks the ones that have taken part in the global optimization algorithm
and {\em expanders} the ones that 
have been incrementally added by optimizing singularly their coordinates. Since common nodes randomly select a collection of landmarks which includes primary landmarks and expanders.

We could assume that these secondary added landmarks
are the cause of our system inaccuracy on short path lengths.
Actually, regular users in the system randomly select a collection of landmarks which 
is the combination of primary landmarks and expanders to calibrate their coordinates. 
Thus, if expanders carry some error they will propagate it along regular nodes, 
resulting in an inaccurate embedding system.    

In order to disproof this hypothesis holds, we experimentally answer the following question:
{\em is there any difference in accuracy in 
having a two phase landmark coordinate computation compared to a single global optimization?}
Figure~\ref{fig:basicare} shows that as we increase the number of primary landmarks the accuracy 
of the system does not variate. 
Thus, our two phase approach (i.e. $16$ primary landmarks and $84$ expanders) 
compared to a single global optimization strategy (i.e.  $100$ primary landmarks and $0$ expanders) does 
not degrade the system accuracy, meanwhile reducing 
the computational complexity of the bootstrap phase.  
%Can we improve the accuracy of shorst distance by improving the accuracy of landmarks? There are tow possible approaches. One is to improve the accuracy of landmarks because every node computes its coordinate based on landmarks. Another method is to add short distance information into coordinate compuation method for a node. 
%
%Based on our observation in~\ref{fig:16land}, we find that basic landmarks have higher accuracy than secondary landmarks. This is because the coordinates of secondary landmark is based on basic landmark which will generate higher errors than what they use. This observation motivates us to increase the number of basic landmarks to improve accuracy. 
%
%However, Figure~\ref{fig:basic} and Figure~\ref{fig:basicare} shows that as we increase the number of basic landmark, the accuracy of secondary landmarks and the average relative error will not changes a lot. That means, Simplex Downhill already gives us the optimal results and we can not get more improvement by change landmark computation method. (Note that the relative error in Figure~\ref{fig:basic} is the average error of distances between all pairs of secondary landmarks.).

Summarizing, we validate that landmark coordinate computation is not the source of error 
in our embedding system and so we need to decrease the error on short distances  
based on a different intuition, which we explore in the next section.  
% in order to improve accuracy on short distance 
%estimation we need to add short distance information into coordinate computation.
%%Thus, the only way left to us is to add short distance information into coordiante computation. 
%Figure~\ref{fig:basicare} implicates that two phase landmark computation method does 
%not degrade the system accuracy compared to one phase landmark computation (basic landmark is $100$ and $0$ expanders). 
%A further understanding lays in the possibility to iteratively use coordinates of other nodes instead of landmarks 
%for regular node coordinate computation. 
%Furthermore, considering that $1$-hop friends information is available in social graphs and is short distance information, we would like to use 1-hop neighbors into computation for improving short distance accuracy in section~\ref{sec:1hop}.

\subsection{Increasing Accuracy with Local Information}
\label{sec:1hop}
The goal of this section is to investigate a practical strategy to improve 
short distance estimation. As we mentioned above, we believe that during
the coordinates computation of common nodes we miss out some basic information. 
Thus, in this section we first intend to investigate the entity of this missed information 
and then explore a strategy to integrate those. 

We observe that the majority of nodes, during their coordinate computation, only use landmarks  
far away from themselves, which means they calibrate their coordinates with long distance information. 
%Contrariwise, almost none use close by landmarks. 
Based on this findings we identify that we are missing {\em local information}, 
that is, short distance references when nodes calibrate their coordinates.  

Here, we intend to explore how to leverage {\em local information}  to 
improve the short distance estimates in our system. Considerring that $1$-hop neighbor information is free, 
We introduce local information in the nodes' coordinates computation
by placing some of their $1$-hop neighbors in substitution of some of those far away landmarks.
Note that these $1$-hop neighbors need to already have their coordinates to be able to substitute landmarks.
Thus, to achieve this goal we design a novel node insertion algorithm, {\em Cascade input order}, 
which guarantees that each node can use some of its $1$-hop neighbors as landmarks, 
because they already have their coordinates. 


%that during the coordinate computation phase of a node it has some neighbors,
%already with their coordinate, to act as landmarks.
%
%The {\em Cascade input order} algorithm iteratively assigns coordinates to a node such that it is guaranteed that 
%each node can use some of its $1$-hop neighbor as landmarks, because they already have their coordinates.  
%In order to integrate local information in optimization algorithm that
%generates node coordinate we provide an algorithm that through an intelligent node  )

% The scheme to use 1-hop friends is straightforward which is shown in Algorithm~\ref{alg:1hop}. We set that, except landmarks, each node can use at most $n$ 1-hop friends into its coordinate computation. Thus, when a node starts to compute its coordinates, it will check the number $m$ of its 1-hop friends already with
% their coordinates at first. If $m$ is larger than $n$, we will randomly select $n$ out of the $m$ nodes; otherwise, we select all the $m (n \geq m \geq 0)$  1-hop friends as its neighbors. Then, the rest neighbors are randomly chosen from landmarks. 
%


%We achieve this goal in tree steps:  first, we explore a systematic 
%manner to guarantee that each node that compute its coordinates can
%leverage local information, reported under {\em Cascade Input Order}
%approach. Then we compare against an approach with absolutely no local information,
%which we call {\em No $1$-hop Landmarks}.
%Finally, we present an intermediate approach between these two extreme 
%named {Mixed landmark distances}, that provides small error on 
%short distance without loose much accuracy in the long distances.  

\begin{figure}[t]
\centering
   \includegraphics[scale=0.65]{figures/egy-cas-diffnei.eps}
   \caption{Average absolute error of Cascade input order with different local landmarks on Egypt graph.}
   \label{fig:egynei3}
\end{figure}
%
%The high level idea behind our implementation, as shown in Algorithm~\ref{alg:1hop}, is that each node should use the position 
%of its $1$-hop friend in place of the official landmarks. Obviously when a node can not 
%replace all the landmark , that already have coordinated,
%it will use randomly selected landmark. In order to the number of $1$-
%hop friends that already have coordinates we design an node input order insertion 
%into the geometric space, named {\em Cascade input order}.

\para{Cascade Input Order Algorithm.} 
This approach is based on the intuition of propagating coordinates starting from the landmarks. 
Banally, the landmarks neighbors can directly use landmarks as their local information, 
which translates in $1$-hop nodes which act as landmarks, named {\em local landmarks}. Iteratively, 
nodes at two hops from landmarks can use the landmark $1$-hop neighbors as their local landmarks, and so on. 
Thus,
each node substitutes some of the landmarks with some of its $1$-hop neighbors, that already have coordinates, 
to introduce local information in the coordinate computation. 

The goal of the Cascade Input Order algorithm design, 
as reported in Algorithm~\ref{cascade}, is to guarantee that each 
node has the maximum number of neighbors with coordinates that can be used as {\em local landmarks}.
The main idea behind this algorithm lays in flooding coordinates through BFS trees rooted on 
landmarks. Note that we don't need to pay the price of computing BFS trees, at this point, 
because they have already been computed during the system bootstrap phase.


%the distances from landmarks to all other nodes, which is equal to build BFS trees from landmarks. 
%Equally, every nodes  knows their distances to all the landmarks and so for each node we define 
%its insertion order as the minimum of its distances to all the landmarks. 
%This input nodes order, to compute coordinates, can be visualized as a cascade which propagates across
%these BFS trees.  This strategy guarantees that every node has at least one $1$-hop friend substituting a landmark. 

\begin{algorithm}
\caption{Cascade Input Order with $n$ $1$-hop local landmarks.}
%\label{alg:1hop} 
\begin{algorithmic}
\STATE //Input: Distances between nodes and landmarks; Neighbors of nodes
\STATE //Output: $k$ neighbors with at most $n$ 1-hop friends
\STATE //Decide nodes input order based on their distances to landmarks
\FOR {each node}
\STATE Find its smallest distances to landmarks;
\STATE Set this distance as its input level $l$;
\ENDFOR

\FOR {each level}
\STATE node in this level will randomly join system;
\STATE node select at most $k$ neighbors from all its neighbors with coordinates to compute its coordinates;
\ENDFOR
\end{algorithmic}\label{cascade}
\end{algorithm}

Figure~\ref{fig:egynei3} shows the average absolute error of Cascade Input Order 
algorithm for different path lengths with different number 
of local landmarks. We investigate different number of local landmarks to explore the 
sensitivity of our system to local information.
Increasing the number of $1$-hop Landmarks from zero to four, the error of 
shortest paths of length $1$ is reduced in average from 
$2.8$ to $0.4$ and $2$-hop shortest path lengths 
decreases from $1.4$ to $0.5$.

Although, we proved that local information are extremely valuable in 
reducing the error on short path lengths, 
the accuracy of long path length seems to degrade as more landmarks we use.
Note that when we use $4$ local landmarks, a quarter of the landmarks are selected as local 
which strongly bias the heterogeneity from short to long distances toward the short ones. 
Therefore, the resulting degradation of long distance estimations is due to the lack of enough  
long distance landmarks. In Figure~\ref{fig:egynei3}  the absolute error of long path 
lengths goes from $0.5$ with no local landmark up to $2.3$ with $4$ local landmark strategy. To make a tradeoff between the accuracy of long disntance and the accuracy of short distance, we implement our system with {\em one} $1$-hop local landmarks and called it as Rigel. To make a distinguishment, we call the system without local landmarks as Raw Rigel.
% Therefore, this result motivate us to design a strategy which mitigates the degradation 
% that local landmarks produce on long distances meanwhile maintaining the advantage found on short distances. 


==> related.tex <==
\section{Related Work}
\label{sec:related}
%In this section, we provide related scientific contributions both in the field of embedding system that on  
%the protocols and applications that can benefit from our system.

%\para{Embedding Systems.} 
%Many embedding systems have been focused on Euclidean Space and 
%Spherical Space. Investigations as~(\cite{small_distortion}, 
%\cite{GNP},~\cite{Vivaldi},~\cite{pic},~\cite{BBS_Euclidean},~\cite{Morphing_sherical}) 
%differ from us in tree important points. First, their design is based on 
%Euclidean space instead we use an Hyperbolic space; second, they focus 
%on small scale Internet graphs and we investigate large scale social 
%graphs; and third, they optimize the functionality of the system on its 
%accuracy meanwhile focus on efficiency and parallelization.

%Rao proposed an Euclidean embedding on planar graphs and
%trees~(\cite{small_distortion}). In Network Coordiante(NC) systems, banch of
%works, e.g. GNP~(\cite{GNP}),
%Vivaldi~(\cite{Vivaldi}), PIC~(\cite{pic}), BBS~(\cite{BBS_Euclidean})
%and so on, map Internet into
%Euclidean. The first work on OSN graph embedding, Orion, is also in
%Euclidean  space. Spherical space are mainly employed in computer
%vision, e.g. ~\cite{Morphing_sherical}. Vivaldi also explored
%Spherical embedding. 

In addition to prior work discussed in Section~\ref{sec:back}, we 
briefly summarize here other related projects focused on social applications 
and social network measurements.

%There are a few embedding systems that use Hyperbolic spaces in the 
%context of network coordinates for Internet 
%graphs~(\cite{Crowcroft_IMC05, BBS_Hyperbolic, Vivaldi_hyperbolic}).
%~\cite{Crowcroft_IMC05, BBS_Hyperbolic,Vivaldi_hyperbolic}. Kleinberg~(\cite{Geo_routing_hyperbolic})
%designed an Hyperbolic embedding algorithm in ad hoc. Also, Some work
%on well structured graphs were explored
%in Hyperbolic Space~(\cite{labeling_hyperbolic}). But different from
%our efficiency-driven system, all these work try to improve accuracy
%without considering implement on massive data. 
%Finally there are two predecessors of embedding system in social 
%graphs~(\cite{shortpath}, \cite{orion10}), where both operate on 
%Euclidean space and only optimize for accuracy. For a more detailed taxonomy of embedding spaces refer to Section~\ref{sec:back}.

\para{Shortest-path based Applications.}
Recently, social networks have inspired a numerose security protocols and social applications in a number of fields. 
In addition to the applications presented in Section~\ref{sec:app}, there are many other social applications based on shortest path
length. For instance, information dissemination~\cite{fast_max_influ} can leverage distances
between nodes to find the most influential nodes. Community detection algorithms on social graphs (see taxonomy from~\cite{santo10})
can benefit from shortest path distances between nodes to classify them in different
clusters. Furthermore, Sybil attack detections are in essence based on community
detection strategies~\cite{sybil10} which make them suitable candidates to leverage our system. 
Neighborhood function~\cite{anf02} uses node distance distribution to predict whether two
graphs are similar or not. Mutual friends detection computes the mutual friends between social users. In~\cite{overstock}, the
auction site calculates social distances to identify
items auctioned within social circle defined by users. All these
applications are based on shortest path computations, therefore, in
essence, they can benefit from our system exactly as the
application presented in Section~\ref{sec:app}.

\para{Studies of Online Social Networks.}
In recent year, there are several impressive researches on understanding
the structure of OSN. As far as we know, Mislove~\cite{mislove07}
published a comprehensive paper to analyze data crawled from Flickr,
Livejournal, Orkut and Youtube. Wilson proposed interaction graphs to
analyze OSN and measured the data crawled from
Facebook~\cite{interaction}. ~\cite{jiang10} uses the same methodology
to measure Renren graph of 43 million users.  Twitter, another famous
OSN was analyzed in ~\cite{twitter_media}. Also there are some other graph
analysis works that use the data gathered from network level to model user
behavior, such as,~\cite{fabricio09,fabian09}. 


